Explaining Inference Queries with Bayesian Optimization

Obtaining an explanation for an SQL query result can enrich the analysis experience, reveal data errors, and provide deeper insight into the data. Inference query explanation seeks to explain unexpected aggregate query results on inference data; such queries are challenging to explain because an explanation may need to be derived from the source, training, or inference data in an ML pipeline. In this paper, we model an objective function as a black-box function and propose BOExplain, a novel framework for explaining inference queries using Bayesian optimization (BO). An explanation is a predicate defining the input tuples that should be removed so that the query result of interest is significantly affected. BO - a technique for finding the global optimum of a black-box function - is used to find the best predicate. We develop two new techniques (individual contribution encoding and warm start) to handle categorical variables. We perform experiments showing that the predicates found by BOExplain have a higher degree of explanation compared to those found by the state-of-the-art query explanation engines. We also show that BOExplain is effective at deriving explanations for inference queries from source and training data on a variety of real-world datasets. BOExplain is open-sourced as a Python package at https://github.com/sfu-db/BOExplain.

==> contents/problem_statement.tex <==
\section{Problem Definition}

In this section, we first define the framework of SQL explanations, and subsequently describe the extension to \sqlml explanations.

\subsection{SQL Explanation}

% f(R, predicate, pipeline1, pipeline2, Q)

% supported query := g(pipeline(R)) -> result

% The meaning of SQL-ML query
% SQL-ML supported query: Q over inference data <- this is what user issues, but needs explanation. Our system needs explanation, what explanation do we look for? Need to define how good our explanation is. Define obj function for some measurement of how good an explanation is. We focus on why the result is higher is expected
% obj func := f( predicate, R, pipeline, Q)

% 1st explain our goal is to find the predicate to min/max result. The introduce obj func
% g has a pipeline from source -> train, train -> inference, Q

% objective function: given data filtered by predicate, return result, find best pred



In this paper, explanations are derived from a single relation $R$; the extension to multiple relations has been formalized in \cite{roy14}. A \textit{numerical query} $Q=E(q_1,\dots,q_k)$ is an arithmetic expression $E$ over queries $q_1, \dots, q_k$ of the form
\begin{align*}
q_i= & \textbf{\textsf{ SELECT}} \text{ agg}(\dots) \textbf{\textsf{ FROM }} R \\
 & \textbf{\textsf{ WHERE }} C_1 \textbf{\textsf{ AND/OR }}\dots\textbf{\textsf{ AND/OR }} C_m
\end{align*}
where agg is an aggregation operation and $C_j$ is a filter condition. The user defines a direction $dir\in\{low, high\}$ indicating how $Q$ should change; $dir=low$ ($high$) means that $Q$ is too high (low). This formulation is used in \cite{roy14}.

\example{Returning to the motivating example in Section~\ref{sec:intro}, the data scientist found that the predicted repeat buyer rate was unexpectedly high. This can be expressed as the numerical query $Q=q_1/q_2$ where
\begin{align*}
    q_1 &= \text{SELECT COUNT * FROM I WHERE M.predict(I)="repeat buyer";} \\
    q_2 &= \text{SELECT COUNT * FROM I;} \\
\end{align*}
Since $Q$ is unexpectedly high, the user sets $dir=low$ to indicate that $Q$ should be minimized.}

An \textit{explanation} for $Q$ is a predicate over a subset of the attributes from $R$. For a numerical attribute $N$, the clause is a range constraint of the form $l\le N\le u$, where $l, u \in [\min(N), \max(N)]$, and $l \le u$. For a categorical attribute $C$, the clause is an equality constraint $C=c$ where $c\in$ domain$(C)$. The final predicate is a conjunction of such clauses, and is formally defined below.

\definition[Explanation]{Given numerical attributes $N_1, \dots, N_n$ and categorical attributes $C_1, \dots, C_m$, an explanation is a predicate $p$ of the form $$p=l_1\le N_1\le u_1\wedge\dots\wedge l_n\le N_n\le u_n\wedge C_1=c_1\wedge\dots\wedge C_m=c_m.$$ The set of all such predicates forms the \textit{predicate space} $S$.}

\example{The source data in Figure~\ref{fig:workflow} contains the attributes Date and Website. An example explanation over these attributes is $$12/01/2020 \le \text{Date} \le 12/10/2020 \wedge \text{Website}=w.$$}

For a predicate $p$, let $\sigma_{\neg p}(R)$ represent $R$ filtered to contain all tuples that do not satisfy $p$. We next formally define SQL explanation.

\begin{definition}[SQL Explanation]
Given a relation $R$, query $Q$, direction $dir$, and predicate space $S$, find the predicate $p\in S$ such that when queries $q_1, \dots, q_k$ are executed on $\sigma_{\neg p}(R)$, $Q$ is minimized if $dir=low$ and maximized if $dir=high$.
\end{definition}


\subsection{\sqlml Explanation}

The difference between SQL and \sqlml explanation is the data over which the explanation is derived. For SQL explanation, the predicate is over the queried relation $R$. However, in the \sqlml setting, an explanation may need to be derived from source, training or inference data, which are defined as follows:
\begin{enumerate}
    \item \textbf{Source data} is data that is in a state not yet ready for feeding into an ML algorithm.
    \item \textbf{Training data} is data that is ready for applying an ML algorithm.
    \item \textbf{Inference data} is data augmented with the model's prediction.
\end{enumerate}

Source data passes through an ML pipeline $\mathcal{P}$ which transforms and featurizes the data to create the  training data. An ML model is fit to the training data, and the ML model predictions are added to the inference data. The queries $q_1, \dots, q_k$ are executed on the inference data. 
% In a SQL-ML query, the user specifies the relation $D\in\{\text{source, training, inference}\}$ from which to derive an explanation.

\begin{figure}
    \centering
    $$f := \begin{cases} f(R, p, \mathcal{P}, M, Q) & \text{if $R$ is source data} \\ f(R, p, M, Q) & \text{if $R$ is training data} \\ f(R, p, Q) & \text{if $R$ is inference data} \\ \end{cases}$$
    \caption{The objective function $f$ with different parameters depending on the data state to derive an explanation}
    \label{fig:obj_func}
\end{figure}

To support a more general query explanation framework, we abstract the numerical query $Q$ into an objective function $f$. The components of the objective function are different depending on the data state from which the explanation is derived. The possible objective functions with corresponding data states are given in Figure~\ref{fig:obj_func}. For each state, the objective function takes as input one relation $R$, a predicate $p$, and a query $Q$. Inside the objective function, $R$ is filtered to consist of all tuples that do not satisfy $p$; let $\sigma_{\neg p }(R)$ represent this relation. Next, if $R$ is source data, $\sigma_{\neg p }(R)$ passes through an ML pipeline $\mathcal{P}$ where it is transformed into training data. Subsequently, a model $M$ is trained, and the query $Q$ is executed on the inference data augmented with the model's predictions. If $R$ is training data, $\sigma_{\neg p }(R)$ is used to train a model $M$, and the query $Q$ is executed on the inference data augmented with the model's predictions. If $R$ is inference data, the query is executed directly on $\sigma_{\neg p }(R)$. The form of $f$ will be clear in the context of the problem. All of $R, \mathcal{P}, M$, and $Q$ are defined by the user (only predicate $p$ is determined by \boexplain), and so we use $f(p)$ as shorthand notation.

% We define the objective function below.

% \definition[Objective function] The objective function $f: (S, R, \mathcal{P}) \rightarrow \mathbb{R}$ filters $R$ by the input predicate, passes $\sigma_{\neg p }(R)$ through $\mathcal{P}$, trains $M$, and executes a query on the results as defined above.

The objective function is optimized in the direction specified by the user. Our query explanation problem is presented formally below.

\begin{definition}[Query Explanation Problem]
Given a predicate space $S$ and objective function $f$, find the predicate that optimizes the objective function:
$$\min_{p\in S}f(p).$$ Use $-f$ if $f$ should be maximized.
\end{definition}


% \section{Problem Definition}\label{sec:prob_def}

% In this section, we define an explanation, the supported queries, and describe our formulation of the query explanation problem as an optimization problem. 

% \subsection{Explanations}

% An \textit{explanation} of a query result is a predicate over a subset of the attributes from the input relation. For a numerical attribute $A$, the clause is a range constraint of the form $l\le A\le u$, where $l, u \in [\min(A), \max(A)]\subset\mathbb{R}$, and $l \le u$. For a categorical attribute $C$, the clause is an equality constraint $C=c$ where $c\in$ domain$(C)$. The final predicate is a conjunction of such clauses, and is formally defined below.

% \definition[Explanation] Given numerical attributes $A_1, \dots, A_n$ and categorical attributes $C_1, \dots, C_m$, an explanation is a predicate of the form $$l_1\le A_1\le u_1\wedge\dots\wedge l_n\le A_n\le u_n\wedge C_1=c_1\wedge\dots\wedge C_m=c_m.$$


% \subsection{Supported Queries}
% This work considers queries on a single relation R that contain one aggregate in the SELECT clause. Specifically, queries of the form
% \begin{align*}
% & \textbf{\textsf{ SELECT}} \text{ agg}(\dots) \textbf{\textsf{ FROM }} R \\
%  & \textbf{\textsf{ WHERE }} C_1 \textbf{\textsf{ AND }}\dots\textbf{\textsf{ AND }} C_m
% \end{align*}
% where $C_i$ is a filter condition, and $m, k \ge 0$.

% Let $M$ be a classification or regression model, and $T$ be the data used to train $M$. $M$.predict($I$) is the model's prediction on an inference relation $I$. We consider the case when the model's prediction appears in the aggregate in the SELECT clause. Incorporating an ML model into other query clauses as defined in \cite{wu2020complaint} is left to future work.

% Finally, to explain a query, the user defines an arithmetic expression over the query results and direction to indicate how the query result should change.


% \example
% Consider a regression model $M$ that predicts income. Suppose the user wants an explanation for why the predicted income is higher for residents in Arizona than in Florida. This can be expressed in our framework with the queries
% \begin{align*}
%     q_1 &= \text{SELECT AVG($M$.predict(I)) FROM R WHERE State=``AZ''} \\
%     q_2 &= \text{SELECT AVG($M$.predict(I)) FROM R WHERE State=``FL''} \\
% \end{align*}
% and that the ratio $q_1/q_2$ should be minimized.

% \subsection{Objective function}\label{sec:obj_func}

% \begin{figure}
%     \centering
%     $$f := \begin{cases} f(R, p, \mathcal{P}, M, Q) & \text{if $R$ is source data} \\ f(R, p, M, Q) & \text{if $R$ is training data} \\ f(R, p, Q) & \text{if $R$ is inference data} \\ \end{cases}$$
%     \caption{The objective function $f$ with different parameters depending on the data state to derive an explanation}
%     \label{fig:obj_func}
% \end{figure}

% To support deriving explanations from data that passes through an ML pipeline, we define the concept of an objective function. The components of the objective function are different depending on the data state from which the explanation is derived. The possible objective functions with corresponding data states are given in Figure~\ref{fig:obj_func}. For each state, the objective function takes as input one relation $R$, a predicate $p$, and a query $Q$. Inside the objective function, $R$ is filtered to consist of all tuples that do not satisfy $p$; let $\sigma_{\neg p }(R)$ represent this relation. Next, if $R$ is source data, $\sigma_{\neg p }(R)$ passes through an ML pipeline $\mathcal{P}$ where it is transformed into training data. Subsequently, a model $M$ is trained, and the query $Q$ is executed on the inference data augmented with the model's predictions. If $R$ is training data, $\sigma_{\neg p }(R)$ is used to train a model $M$, and the query $Q$ is executed on the inference data augmented with the model's predictions. If $R$ is inference data, the query is executed directly on $\sigma_{\neg p }(R)$. The form of $f$ will be clear in the context of the problem. All of $R, \mathcal{P}, M$, and $Q$ are defined by the user (only predicate $p$ is determined by \boexplain), and so we use $f(p)$ as shorthand notation

% We define the objective function below.

% \definition[Objective function] Let $S$ be the set of all predicates. The objective function $f: (S, R, \mathcal{P}) \rightarrow \mathbb{R}$ filters $R$ by the input predicate, passes $\sigma_{\neg p }(R)$ through $\mathcal{P}$, trains $M$, and executes a query on the results as defined above.

% The objective function is optimized in the direction specified by the user. Our query explanation problem is presented formally below.

% \definition[Query Explanation Problem] Given a predicate space $S$ and objective function $f$, find the predicate that optimizes the objective function:
% $$\min_{p\in S}f(p).$$ Use $-f$ if $f$ should be maximized.

% given table and search columns, objective function (scores each predicate) input table, output score. Find a predicate such that after apply the predicate you get a new table, and feeding it into the objective function,
%goal find predicate such that when we move tuples from the data that satisfy the pred, and feed into obj func, the score is optimized

%coarse-grained: given table, find predicate such that score function is optimized
% score function takes as input filtered table

% \newpage



% \textbf{Section 2 outline: }
% \textit{Problem Defintion}
% \begin{enumerate}
% \item \textit{Explanations}
% \begin{enumerate}
%     \item An explanation is a predicate in the form of a conjunction of equality constraints on categorical variables and range constraints on numerical variables, where each variable appears once in the predicate
%     \item Give example
% \end{enumerate}
% \item \textit{Supported queries}
% \begin{enumerate}
%     \item \textit{SQL-only queries }
%     \begin{enumerate}
%         \item Follow Scorpion and Suciu query setup.
%     \end{enumerate}
%     \item \textit{SQL-ML queries}. Follow Rain's Query 2.0 paradigm. Clearly define what an explanation is in the three settings:
%     \begin{enumerate}
%         \item inference data
%         \item training data
%         \item source data
%     \end{enumerate}
% \end{enumerate}
% \item \textit{The objective function}. Optimization problem studied in the paper. Arithmetic expression over query results, and direction indicating the value is too low or high
% \end{enumerate}

% \textbf{Section 4 outline:}
% \textit{The \boexplain Framework}
% \begin{enumerate}
% \item \textit{Framework overview}
% \begin{enumerate}
%     \item Break our system up into parts, e.g., preprocessor, candidate selector, and explanation evaluator. Use a figure (currently Figure~\ref{fig:boexplain}) to step through each part
% \end{enumerate}
% \item \textit{Parameters and their domain}. How we model our problem into a suitable form for BO
% \item \textit{API design}
% \begin{enumerate}
%     \item Overview and explanation. Discuss how we make it easy
%     \item show how to use our API to explain different queries
% \end{enumerate}
% \end{enumerate}

% \textbf{Section 5 outline:}
% \textit{How to handle categorical variables}
% \begin{enumerate}
% \item Individual contribution encoding
% \item Frequency encoding
% \end{enumerate}

% \textbf{Section 6 outline:}
% \textit{How to handle invalid predicates}
% \item Introduce the concept of a BO problem
% \begin{enumerate}
%     \item What is the BO problem
%     \item Exploration vs exploitation
%     \item Surrogate model
%     \item Acquisition function
% \end{enumerate}
% \item Define \boexplain in terms of the input (single data table, user-defined columns over which to find the predicate, and objective function) and output (predicate). See Algorithm~\ref{algo:boexplain}.
% \item Example use cases:
% \begin{enumerate}
%     \item ML source data debugging (see Algorithm~\ref{algo:source_debug})
%     \item ML training data debugging
%     \item Typical SQL explanation.
%     \begin{itemize}
%         \item Explain here the queries we support (basically the beginning of Section 2 \cite{roy14})
%     \end{itemize}
% \end{enumerate}

% \begin{algorithm}
%   \caption{\boexplain}
%   \label{algo:boexplain}
%   \DontPrintSemicolon
%   \SetKwFunction{FMain}{BOExplain}
%   \SetKwProg{Fn}{Function}{:}{}
%   \SetKwBlock{Repeat}{repeat}{}

%   \KwIn{Relation $R_i$ \bl{Here $R_i$ can be a base relation or a training dataset. Is this confusing?}, search attributes $(A_{i_1}, \dots, A_{i_n})$ of $R_i$, objective function $f$}

%   \Fn{\FMain{$R_i, (A_{i_1},\dots,A_{i_n}), f$}}{
%     Initialize BO($dom(A_{i_1}), \dots, dom(A_{i_n})$)\;
%     \Repeat{
%         \textit{p} $\leftarrow$ BO.suggest\_predicate()\;
%         $R_i' \leftarrow$ remove tuples satisfying \textit{p} from $R_i$\;
%         \textit{score} $\leftarrow f(R_i')$\;
%         BO.update(\textit{predicate, score})\;
%     }
%     \KwRet BO.best\_predicate()\;
%   }
% \end{algorithm}

% \begin{algorithm}
%   \caption{Source data debugging objective function}
%   \label{algo:source_debug}
%   \DontPrintSemicolon
%   \SetKwFunction{FMain}{f}
%   \SetKwProg{Fn}{Function}{:}{}
%   \SetKwBlock{Repeat}{repeat}{}

%   \KwIn{Relations $R_i,\dots,R_n$, inference data $I$}

%   \Fn{\FMain{$R_1, \dots, R_n$, $I$}}{
%     T $\leftarrow$ Construct($R_1, \dots, R_n$)\;
%     M $\leftarrow$ Train(T)\;
%     I $\leftarrow$ Predict(M, I)\;
%     q $\leftarrow$ Query(I)\;
%     \KwRet q\;
%   }
% \end{algorithm}



% In this section, we formalize the problem, state the supported queries, and discuss why and how BO can be applied to the query explanation problem.

% \subsection{Framework}

% Consider a database $D$ with $k$ relations $R_1,\dots,R_k$. We follow the explanation setup in Roy and Suciu \cite{roy14}. Let queries $q_1,\dots,q_m$ be Select Project Join Aggregate (SPJA) queries on $D$ containing one aggregation function, and $$Q=E(q_1,\dots,q_m)$$ be an arithmetic expression containing operators such as $+,-,\cdot,\div,\exp,\log$ etc. The user's question is of the form $(Q, dir)$ representing whether $Q$ is too high or too low.


% We extend this framework to support queries embedded with one or more ML models; we follow the queries supported in Rain \cite{wu2020complaint}. Let $T$ be the training dataset for model $M$ derived from $D$. We allow a model to appear in the SELECTION, WHERE, and GROUP BY clauses. As before, we can then execute queries $q_1, \dots, q_m$ (possibly containing an ML model), and finally express a question $Q=E(q_1,\dots,q_m)$. 


% This framework enables \boexplain to provide an explanation for all queries supported in previous system. However, the efficacy at finding a solution in each problem setting is unknown. 

% \subsection{Explanation}

% An explanation is a predicate composed of a conjunction of range constraints on numerical variables and equality constraints on categorical variables, where each variable appears once in the predicate. We borrow this definition of explanation from prior work \cite{wu13, roy14, abuzaid2020diff} More precisely, given categorical attributes $C_1, C_{n_c}$ and numerical attributes $N_1\dots N_{n_r}$ a predicate is of the form $$C_1=c_1\wedge\dots\wedge C_{n_c}=c_{n_c}\wedge a_1\le N_1\le b_1\wedge\dots\wedge a_{n_n}\le N_{n_n}\le b_{n_n}$$
% In \boexplain, the user specifies $m$ categorical and/or numerical attributes $A_i,\dots,A_m$ on a single relation $R_j\in D$ or the training relation $T$, and \boexplain returns a predicate with $m$ clauses, ie one constraint for each variable.

% \section{Problem Statement}

% Given $(Q, dir)$, $A_1,\dots, A_m$, \boexplain seeks to find a predicate such that removing tuples that satisfy the predicate from the input dataset that reverses the trend of the dir.

==> contents/removed_contents.tex <==
We propose to model the predicate search problem as a hyper-parameter tuning problem, where the predicate constraints are the parameters. A range constraint is used for a numerical columns and an equality constraint is used for a categorical column. The constraint values can be learned by modelling how they effect the quality of an explanation. Bayesian optimization (BO) is a widely used method for finding the global optimum of a black-box function. The principle idea behind BO is to balance exploration and exploitation of the search space: exploration is the tendency of the algorithm to search unexplored areas, and exploitation is the component of the algorithm that continually investigate promising regions. BO has been proven to work in many scenarios to optimize an objective function \cite{}.


This framework can address the aforementioned limitations of the previous work: since BO is a global function optimizer, it can explain the results of many aggregate queries, including complex UDFs with perhaps ML models. Also, BO is an iterative algorithm, and can hence progressively return better and better explanations to the user. 
